Fact-Level Confidence Calibration and Self-Correction

Confidence calibration in LLMs, i.e., aligning their self-assessed confidence with the actual accuracy of their responses, enabling them to self-evaluate the correctness of their outputs. However, current calibration methods for LLMs typically estimate two scalars to represent overall response confidence and correctness, which is inadequate for long-form generation where the response includes multiple atomic facts and may be partially confident and correct. These methods also overlook the relevance of each fact to the query. To address these challenges, we propose a Fact-Level Calibration framework that operates at a finer granularity, calibrating confidence to relevance-weighted correctness at the fact level. Furthermore, comprehensive analysis under the framework inspired the development of Confidence-Guided Fact-level Self-Correction ($\textbf{ConFix}$), which uses high-confidence facts within a response as additional knowledge to improve low-confidence ones. Extensive experiments across four datasets and six models demonstrate that ConFix effectively mitigates hallucinations without requiring external knowledge sources such as retrieval systems.

==> 5_exp.tex <==
\section{Experiment}



\subsection{Experiment Setup}
This section outlines the experimental setups, including the datasets, models, and evaluation.

\paragraph{Datasets} We employ two datasets:
(1) LongFact~\cite{wei2024long}: A dataset consisting of prompts designed to assess a model's factuality in long-form responses created by GPT-4.
(2) ASQA~\cite{stelmakh2022asqa}: A dataset designed for long-form question answering that uniquely centers on ambiguous factoid questions.

\paragraph{Models} 
We use five models from different families and scales to validate our method, including:
(1) Llama~\cite{DBLP:journals/corr/abs-2307-09288}: include Llama-7b-chat and Llama-13b-chat.
(2) Vicuna~\cite{vicuna2023}: include Vicuna-7b and Vicuna-13b.
(3) GPT~\cite{DBLP:conf/nips/BrownMRSKDNSSAA20}: GPT-3.5-turbo.

\paragraph{Correctness and Relevance Evaluation} 
For correctness and relevance evaluation, we use the Search-Augmented Factuality Evaluator (SAFE), which is a pipeline proposed by~\cite{wei2024long} that employs LLMs as agents to automatically evaluate the factuality of long-form responses. It utilizes a multi-step reasoning process that includes sending search queries to Google Search~\cite{hillis2012google} to verify the information provided. 
For the fact correction evaluation, we use GPT-4 for zero-shot pair-wise evaluation (see prompts in Appendix~\ref{app:prompts}).

\paragraph{Evaluation Metrics}
For calibration evaluation,  we use Expected Calibration Error (ECE)~\cite{guo2017calibration,Naeini2015ObtainingWC} at the response-level, and our F-ECE at the fact-level as introduced in~\cref{calibration metric}.
For self-correction evaluation, the evaluation metrics are twofold. Firstly, we use Accuracy, Precision, and Recall~\cite{powers2020evaluation} to evaluate error detection. Then, we use improvement ratio, same ratio, and regression ratio to evaluate self-correction.

\subsection{Results for Fact-Level Calibration}

This section provides detailed implementation and comprehensive experiment results of our fact-level calibration framework. As introduced in~\cref{sec:observations}, we have three key observations.


\begin{table}[h]
\renewcommand{\arraystretch}{0.3}
\centering
\caption{Comparison of response-level and our fact-level calibration performance of five base models in terms of (F-)ECE under ASQA and LongFact datasets.}
\label{tab:ece}
\begin{adjustbox}{width=\linewidth}
\setlength{\tabcolsep}{3mm}
\begin{tabular}{lccc}
\toprule
Base Model & Method & ASQA & LongFact \\
\midrule
\multirow{2}{*}{Llama-2-7b} &  Fact & 0.261 & 0.211\\ 
\cmidrule(lr){2-4}
&  Response & 0.251 & 0.141 \\ 
\cmidrule(lr){1-4}
\multirow{2}{*}{Llama-2-13b} & Fact  & 0.240 & 0.156 \\ 
\cmidrule(lr){2-4}
& Response  & 0.261 & 0.131 \\ 
\cmidrule(lr){1-4}
\multirow{2}{*}{Vicuna-7b} & Fact & 0.337 & 0.151\\ 
\cmidrule(lr){2-4}
& Response & 0.352 & 0.137 \\ 
\cmidrule(lr){1-4}
\multirow{2}{*}{Vicuna-13b} & Fact  &  0.254 & 0.113 \\
\cmidrule(lr){2-4}
& Response & 0.269 & 0.109 \\ 
\cmidrule(lr){1-4}
\multirow{2}{*}{GPT-3.5-turbo} & Fact & 0.179 & 0.086 \\ 
\cmidrule(lr){2-4}
& Response & 0.185 & 0.094\\ 
\bottomrule
\end{tabular}
\end{adjustbox}
\end{table}


\begin{figure*}[t]
    \centering
    \includegraphics[width=\linewidth]{pic/exp-violin.pdf}
    \caption{Comparison of confidence distribution across different responses between fact-level and response-level. The purple are our fact-level distribution under different statistical metrics, the gray is the response-level distribution.}
    \label{fig:exp-violin}
\end{figure*}

\paragraph{Calibration Comparison for Observation 1}
For Observation 1, we compare our fact-level and response-level calibration in accordance with the protocol in~\cite{guo2017calibration}. We illustrate reliability histograms and compute the summary statistics of ECE and our F-ECE to evaluate calibration.
The procedures are implemented as follows:
For fact-level, we evaluate confidence, correctness, and relevance as described in~\cref{sec:cal_frame}.
For response-level, we use a verbalization-based method following the procedure in~\cite{huang2024calibrating}, where the model is prompted to provide a single confidence score for the whole response. For a detailed prompt template, please refer to Appendix~\ref{app:prompts}.
For the reliability histogram, we divided the model's predictions into ten bins based on the confidence score and calculated the average accuracy for each bin.
From the perspective of the histogram, an optimally calibrated model should have its bar graph in a diagonal shape to achieve the smallest gap area. 
The results are depicted in~\cref{fig:ob-hist} and~\cref{tab:ece}. 


\paragraph{Across-Responses Confidence Distribution for Observation 2}

For Observation 2, we examine how our fact-level calibration can mitigate the over-confidence issue by analyzing the distribution of confidence scores.
The procedures are implemented as follows:
For the response-level, we use a verbalization-based method to obtain a score for each response and visualize its distribution across the entire dataset using violin plots.
For the fact-level, since the confidence for a single response is represented as a vector rather than a scalar, we compute three different statistical measures: the mean, maximum, and minimum of the vector. We then visualize these measures as three separate violin plots.
The results are depicted in~\cref{fig:exp-violin}. 



\begin{figure*}[t]
    \centering
    \includegraphics[width=\linewidth]{pic/exp-box.pdf}
    \caption{Confidence distribution within responses at the fact level, the red bar is the response-level score.}
    \label{fig:exp-box}
    \vspace{-4mm}
\end{figure*}


\paragraph{Within-Responses Confidence Distribution for Observation 3}
For Observation 3, we investigate the variance in fact-level confidence within individual responses.
The procedures are implemented as follows:
For each response, we obtain its confidence vector and visualize its distribution using box plots. Due to space limitations, we have visualized 10 responses for each model in each dataset in~\cref{fig:exp-box}, whereas this number is 50 in~\cref{fig:ob-box}. The red bar is the confidence score of the whole response at response-level.




\subsection{Results for Self-Correction}

\paragraph{Error Detection}
\cref{tab:detect} presents the error detection results of our proposed method based on five different base models. It can be seen that, in terms of Accuracy and Precision, larger models perform better than smaller models, i.e., GPT > 13b > 7b. However, all models somewhat fall short in Recall, indicating that many erroneous facts are not being detected. This suggests that all models exhibit a certain degree of overconfidence, often considering incorrect answers to be correct.


\paragraph{Error Correction}
\cref{tab:self_correction} presents the error correction results of our proposed method based on five different base models. It can be seen that, among the three outcomes "improve," "same," and "regress," our method achieves the highest proportion of "improve" for all models except LLaMA. This indicates that our method effectively enables the models to self-correct and achieve better generation results.


\begin{table}[h]
\centering
\caption{Acc., Precision and Recall of error-detection.}
\label{tab:model_comparison}
\begin{adjustbox}{width=\linewidth}
\setlength{\tabcolsep}{1mm}
\begin{tabular}{lccc}
\toprule
Base Model & Accuracy (\%)  & Precision (\%)  & Recall (\%)  \\ 
\midrule
GPT-3.5-turbo & 83.29 & 87.89 & 13.71 \\ 
Vicuna-7b & 60.06 & 99.90 & 0.15  \\ 
Vicuna-13b & 74.81 & 77.68 & 8.46 \\ 
Llama-2-7b & 64.26 & 67.86 & 13.35\\ 
Llama-2-13b & 70.45 & 77.45 & 30.62\\ 
\bottomrule
\end{tabular}
\label{tab:detect}
\end{adjustbox}
\end{table}


\begin{table}[h]
\centering
\caption{GPT-4 evaluation of the self-correction.}
\label{tab:model_comparison}
\begin{adjustbox}{width=\linewidth}
\setlength{\tabcolsep}{1mm}
\begin{tabular}{lcccc}
\toprule
Base Model & Improved (\%) & Same (\%)& regressed (\%) & \#revised\\ 
\midrule
GPT-3.5-turbo & 46.30 & 24.07 & 29.63 & 108 \\ 

Vicuna-7b & 50.00  & 50.00 & 0.00 & 2 \\ 
Vicuna-13b & 49.40 & 28.92 & 21.69 & 83 \\
Llama-2-7b & 6.76 & 12.56 & 80.68 & 207 \\ 
Llama-2-13b & 53.35 & 19.59 & 27.07 & 418\\ 
\bottomrule
\end{tabular}
\label{tab:self_correction}
\end{adjustbox}
\vspace{-2mm}
\end{table}

\section{Conclusion}

This paper introduces a novel fact-level calibration framework to address hallucination issues in long-form responses generated by LLMs. Traditional single-estimate confidence methods are inadequate for complex outputs with multiple facts. By evaluating each fact's correctness and relevance individually, both externally and internally, our framework enables fine-grained confidence assessments. It sets a higher standard than response-level approaches, mitigates over-confidence, and reveals significant confidence variance among facts within responses. Leveraging high-confidence facts for in-context learning effectively mitigates hallucination, as validated across multiple datasets and models.
